Protection of quantum information in a chain of Josephson junctions

Symmetry considerations are key towards our understanding of the fundamental laws of Nature. The presence of a symmetry implies that a physical system is invariant under specific transformations and this invariance may have deep consequences. For instance, symmetry arguments state that a system will remain in its initial state if incentives to actions are equally balanced. Here, we apply this principle to a chain of qubits and show that it is possible to engineer the symmetries of its Hamiltonian in order to keep quantum information intrinsically protected from both relaxation and decoherence. We show that the coherence properties of this system are strongly enhanced relative to those of its individual components. Such a qubit chain can be realized using a simple architecture consisting of a relatively small number of superconducting Josephson junctions.

==> supplementary_from_paul_1.tex <==
\setcounter{page}{1}

\section*{Supplementary Material}

\subsection*{Disorder}

In order to model the effect of disorder on our qubit we vary the junction charging and tunneling energies, loop areas and gate charges as described in the main body of the text. In Fig. \ref{fig:junction_disorder} we display the effect of $2 \%$ disorder in the junction parameters and we find the good performance of the qubit is retained.

In Fig. \ref{fig:loop_disorder} we turn our attention to disorder in the loops of the circuit by introducing a $0.2 \%$ variation in their sizes. Such disorder does not affect the charge noise dephasing time, so we only display the flux noise dephasing time and the gap of the qubit. We find that our design is robust to this level of disorder with no significant change in the gap and even a slight improvement in flux dephasing time.

Finally in Fig. \ref{fig:gate_disorder} we introduce gate charge disorder at a level of $0.1 \%$. This kind of disorder does not affect the flux noise dephasing time so we only display the charge noise dephasing time, which now varies significantly. However, the dephasing time remains in the millisecond range and the gap is almost unaffected.

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{junction_disorder_histogram.png}
\caption{\textbf{Junction disorder.} We introduce a $2 \%$ variation in the sizes and oxidation parameters of the junctions and plot histograms of the resulting variations in (\textbf{a}) the charge dephasing time $T^c_\phi$, (\textbf{b}) the flux dephasing time $T^f_\phi$ and (\textbf{c}) the gap of the qubit $\omega_{01}/2\pi$. The resulting expectation values and standard deviations of these characteristics are (\textbf{a}) $2.94 \pm 0.10 ~\mathrm{ms}$, (\textbf{b}) $5.32 \pm 0.54 ~\mathrm{ms}$ and (\textbf{c}) $708 \pm 21 ~\mathrm{MHz}$ respectively. This level of disorder creates no significant degradation in the qualities of the qubit. }\label{fig:junction_disorder}
\end{figure*}

\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{flux_disorder_histogram.png}
\caption{\textbf{Loop disorder.} We introduce a $0.2 \%$ variation in the sizes of the loops and plot histograms of the resulting variations in (\textbf{a}) the flux dephasing time $T^f_\phi$ and (\textbf{b}) the gap of the qubit $\Delta \omega_{01}/2\pi$. The resulting expectation values and standard deviations of these characteristics are (\textbf{a}) $5.45 \pm 0.46 ~\mathrm{ms}$ and (\textbf{b}) $703 \pm 2 ~\mathrm{MHz}$ respectively. This level of disorder creates no significant degradation in the qualities of the qubit. }\label{fig:loop_disorder}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{gate_disorder_histogram.png}
\caption{\textbf{Gate disorder.} We introduce a $0.1 \%$ variation in the gate charges and plot histograms of the resulting variations in (\textbf{a}) the charge dephasing time $T^c_\phi$ and (\textbf{b}) the gap of the qubit $\Delta \omega_{01}/2\pi$. The resulting expectation values and standard deviations of these characteristics are (\textbf{a}) $1.44 \pm 0.78 ~\mathrm{ms}$ and (\textbf{b}) $704.103 \pm 0.001 ~\mathrm{MHz}$ respectively. This level of disorder reduces the coherence time of the qubit but leaves the gap unchanged. }\label{fig:gate_disorder}
\end{figure*}
